Autonomy and Perception for Space Mining

Future Moon bases will likely be constructed using resources mined from the surface of the Moon. The difficulty of maintaining a human workforce on the Moon and communications lag with Earth means that mining will need to be conducted using collaborative robots with a high degree of autonomy. In this paper, we describe our solution for Phase 2 of the NASA Space Robotics Challenge, which provided a simulated lunar environment in which teams were tasked to develop software systems to achieve autonomous collaborative robots for mining on the Moon. Our 3rd place and innovation award winning solution shows how machine learning-enabled vision could alleviate major challenges posed by the lunar environment towards autonomous space mining, chiefly the lack of satellite positioning systems, hazardous terrain, and delicate robot interactions. A robust multi-robot coordinator was also developed to achieve long-term operation and effective collaboration between robots.

==> figures/swerve_drive/swerve-doc.tex <==
\hypertarget{swerve-drive}{%
\section{Swerve Drive}\label{swerve-drive}}

The NASA SRC robots are equipped with four wheels which can be
indepedently driven and steered. This provides a holonomic drivetrain
which presents a unique control problem. We seek to answer the question,
`how do we drive the individual wheels to achieve a desired net linear
or angular velocity?' Assuming an ideal system, inverse kinematics can
be derived to address this problem.

\hypertarget{robot-model}{%
\subsection{Robot Model}\label{robot-model}}

\begin{figure}
\centering
\includegraphics{robot_model.pdf}
\caption{Robot Model}
\end{figure}

Consistent with \href{https://www.ros.org/reps/rep-0103.html}{ROS
coordinate system conventions} we define a right-handed coordinate
system with the X axis as `forward' and the Y axis as `strafe' in a
leftwards direction, from a birds-eye view of the robot. The Z axis
extends out of the page, and angles increase counter-clockwise. The
origin \(O\) is the geometric centre of the robot.

Each wheel is mounted at \(\mathbf{r}_n=(x_n,y_n)\) where
\(\mathbf{r}_n\) is the displacement vector from the centre of rotation
(COR) of the robot to the wheel. In this diagram, the centre of rotation
is also the geometric centre of the robot, although it doesn't have to
be.

\(\mathbf{V}=(v_x,v_y)\) is the (desired) net linear velocity of the
robot at the COR, and \(\omega\) is the (desired) angular velocity about
the COR.

\hypertarget{wheel-model}{%
\subsubsection{Wheel Model}\label{wheel-model}}

Consider one of the four wheels.

\begin{figure}
\centering
\includegraphics{wheel_model.pdf}
\caption{Wheel Model}
\end{figure}

The wheel is inclined at an angle \(\theta\) from the X axis, and is
travelling at net velocity \(\mathbf{v}_n\), which consists of the net
linear velocity \(\mathbf{V}\) and a tangential velocity component
\(\mathbf{v}_{Tn}\) provided by the angular velocity of the robot
\(\omega\).

In three dimensions, the tangential velocity is calculated by
\(\mathbf{v}_{Tn}=\boldsymbol{\omega}\times\mathbf{r}_n\), so

\[
\begin{split}
    \mathbf{v}_{Tn}&=\boldsymbol{\omega}\times\mathbf{r}_n\\
    &=\begin{vmatrix}
        \mathbf{i} & \mathbf{j} & \mathbf{k}\\
        0 & 0 & \omega\\
        x_n & y_n & 0
      \end{vmatrix}\\
    &=\mathbf{i}
      \begin{vmatrix}
          0 & \omega\\
          y_n & 0
    \end{vmatrix}
    -\mathbf{j}
    \begin{vmatrix}
        0 & \omega \\
        x_n & 0
    \end{vmatrix}
    +\mathbf{k}
    \begin{vmatrix}
        0 & 0 \\
        x_n & y_n
    \end{vmatrix}\\
    &= (-\omega y_n,\omega x_n, 0)
\end{split}
\]

which is equivalent to \(\mathbf{v}_{Tn}=(-\omega y_n, \omega x_n)\) in
two dimensions.

The wheel has net velocity
\(\mathbf{v}_n=\mathbf{V}+\mathbf{v}_{Tn}=(v_x,v_y)+(-\omega y_n,\omega x_n)=(v_x-\omega y_n, v_y+\omega x_n)\).

For all four wheel velocities, the control system can then be
represented in matrix form as

\[
\begin{bmatrix}
v_{0x} & v_{0y}\\ 
v_{1x} & v_{1y}\\ 
v_{2x} & v_{2y}\\ 
v_{3x} & v_{3y} 
\end{bmatrix}
=
\begin{bmatrix}
1 & -y_0 & x_0\\ 
1 & -y_1 & x_1\\ 
1 & -y_2 & x_2\\ 
1 & -y_3 & x_3
\end{bmatrix}
\begin{bmatrix}
v_x & v_y\\ 
\omega & 0\\
0 & \omega 
\end{bmatrix}
\]

Equivalently \(V=BU\) where \(V\) is the matrix of outputs, \(B\) is the
control (coefficient) matrix, and \(U\) is the matrix of inputs.

These are the X- and Y-components of the wheel velocity vectors, so the
angle at which to drive wheel \(n\) is given by
\(\theta_n=\mathrm{arctan2}(v_{ny}, v_{nx})\) where \(\mathrm{arctan2}\)
is a quadrant-aware arctangent function, and the linear speed of each
wheel is given by \(v_n=\sqrt{v_{nx}^2+v_{ny}^2}\). This could be
divided by the wheel radius to find the rotational speed of each wheel.

If the COR is at the geometric centre and origin of a rectangular
drivetrain with wheel separations \(2L_1\) and \(2L_2\) as in the Robot
Model diagram, then the model parameters are as follows.

\begin{longtable}[]{@{}cc@{}}
\toprule
\(n\) & \(\mathbf{r}_n=(x_n,y_n)\)\tabularnewline
\midrule
\endhead
0 & \((L_1,L_2)\)\tabularnewline
1 & \((L_1,-L_2)\)\tabularnewline
2 & \((-L_1,-L_2)\)\tabularnewline
3 & \((-L_1,L_2)\)\tabularnewline
\bottomrule
\end{longtable}

The control matrix becomes

\[
B=\begin{bmatrix}
1 & -L_2 & L_1\\
1 & L_2 & L_1\\
1 & L_2 & -L_1\\
1 & -L_2 & -L_1
\end{bmatrix}
\]

Suppose the wheels can individually be driven at a maximum speed of
\(v_{max}\), meaning the maximum value of either \(v_x\) or \(v_y\) is
also \(v_{max}\). Maximum angular velocity occurs when each wheel is
angled 45 degrees and driven at \(v_{max}\) in the same direction,
giving a \(\omega_{max}=\frac{v_{max}}{r}\) where
\(r=\sqrt{L_1^2+L_2^2}=|\mathbf{r}_n|\). The inputs can therefore be
expressed as proportions of these maximum values. Let
\(k_x,k_y,k_\omega\) be between -1 and 1 such that \(v_x=k_xv_{max}\),
\(v_y=k_yv_{max}\), and \(\omega=k_\omega\omega_{max}\). We can use
these to show that

\[
V=v_{max}\begin{bmatrix}
1 & -\frac{L_2}{r} & \frac{L_1}{r} \\[3pt]
1 & \frac{L_2}{r} & \frac{L_1}{r} \\[3pt]
1 & \frac{L_2}{r} & -\frac{L_1}{r} \\[3pt]
1 & -\frac{L_2}{r} & -\frac{L_1}{r} \\[3pt]
\end{bmatrix}
\begin{bmatrix}
k_x & k_y\\ 
k_\omega & 0\\
0 & k_\omega 
\end{bmatrix}
\]

Since \(r=\sqrt{L_1^2+L_2^2}\), \(\frac{L_2}{r}\) and \(\frac{L_1}{r}\)
are simply the ratios of the sides of a right-angled triangle with side
lengths \(L_2\) and \(L_1\) with its hypotenuse.

\begin{figure}
\centering
\includegraphics{triangle.pdf}
\caption{Triangle}
\end{figure}

Let \(\theta=\arctan\frac{L_1}{L_2}\) as in the diagram. Then

\[
V=v_{max}\begin{bmatrix}
1 & -\cos\theta & \sin\theta \\
1 & \cos\theta & \sin\theta \\
1 & \cos\theta & -\sin\theta \\
1 & -\cos\theta & -\sin\theta \\
\end{bmatrix}
\begin{bmatrix}
k_x & k_y\\ 
k_\omega & 0\\
0 & k_\omega 
\end{bmatrix}
\]

We can rewrite \(V=\sin\Theta \cdot U=v_{max}\sin\Theta \cdot K\) where
\[
\Theta=\begin{bmatrix}
\frac{\pi}{2} & \theta-\frac{\pi}{2} & \theta \\
\frac{\pi}{2} & \frac{\pi}{2}-\theta & \theta \\
\frac{\pi}{2} & \frac{\pi}{2}-\theta & -\theta \\
\frac{\pi}{2} & \theta-\frac{\pi}{2} & -\theta \\
\end{bmatrix}
\] and \[
K=\begin{bmatrix}
k_x & k_y\\ 
k_\omega & 0\\
0 & k_\omega 
\end{bmatrix}
\]

So we have managed to characterise the model in terms of a single
constant \(\theta\). We can eliminate \(v_{max}\) by dividing out to get
\(P=\sin\Theta \cdot K\) where \[
P=\begin{bmatrix}
p_{0x} & p_{0y}\\ 
p_{1x} & p_{1y}\\ 
p_{2x} & p_{2y}\\ 
p_{3x} & p_{3y} 
\end{bmatrix}
\] and \(p_n\in[-1,1]\) is the proportion of `effort' applied to the
wheel, with \(|p_n|=1\) corresponding to maximum speed.

We have derived an ideal model whose only physical dependency is the
wheel locations.

\hypertarget{application}{%
\subsection{Application}\label{application}}

Let us redefine the input and output matrices to use complex numbers.
\[\mathbf{p}=\begin{bmatrix}
p_{0x} + ip_{0y}\\ 
p_{1x} + ip_{1y}\\ 
p_{2x} + ip_{2y}\\ 
p_{3x} + ip_{3y} 
\end{bmatrix}
\]

\[\mathbf{k}=\begin{bmatrix}
k_x + ik_y\\ 
k_\omega + i0\\
0 + ik_\omega 
\end{bmatrix}
\]

These are now complex vectors instead of matrices, and we have
\(\mathbf{p}=\sin\Theta\cdot\mathbf{k}\). The output calculations are
simplified to \(\theta_n=\arg(p_{nx}+ip_{ny})\) and
\(p_n=|p_{nx}+ip_{ny}|\). These are much simpler to code using
e.g.~\texttt{numpy} and we get useful characteristics such as
quadrant-aware, bounded arctan for free.

\hypertarget{non-ideal-characteristics}{%
\subsubsection{Non-ideal
Characteristics}\label{non-ideal-characteristics}}

Assuming an ideal model provides freedoms such as instantaneously
changing the wheel angle, however in practice this is not possible. In
particular, consider driving forward at full-speed
\((k_x=1,k_y=0,k_\omega=0)\to(p_{n}=1,\theta_n=0)\), and then
immediately reversing at full speed \((p_{n}=1,\theta_n=\pi)\).
According to this model, we need to turn the wheels 90 degrees to
reverse, whereas we can simply drive them in the opposite direction
without changing the angle. This is a limitation as \(p_n\) is a
positive magnitude, while negative \(p_n\) indicates driving a wheel in
reverse.

Consider a wheel with current velocity \(v\) and desired velocity \(v'\)
as in the following diagram.

\begin{figure}
\centering
\includegraphics{vectors.pdf}
\caption{Vectors}
\end{figure}

The angle \(\phi\) between \(v\) and \(v'\) is greater than 90 degrees,
but the angle between \(v\) and \(-v'\) is much smaller. In this case,
it will be faster to turn the wheel to the angle of \(-v'\) and drive it
in reverse instead of turning to \(v'\) and driving it forward.

In general, \(-v'\) will be closer to \(v\) if the angle between \(v\)
and \(v'\) is greater than 90 degrees. A simple test for this is to test
whether the dot product \(v\boldsymbol\cdot v'\) is negative (this comes
from the formula for cosine of the angle between two vectors).

Thus, we can change the sign of \(p_n\) and the angle of \(\theta_n\)
based on the sign of
\((-p'_{nx}-ip'_{ny})\boldsymbol\cdot(p_{nx}+ip_{ny})=-p'_{nx}p_{nx}-p'_{ny}p_{ny}\)
(complex dot product) and the angle of \(-p'_{nx}-ip'_{ny}\).

Note if the current or future velocity is 0, we can just compare on the
angular positions of the wheels instead of the speeds.

\hypertarget{further-development}{%
\subsubsection{Further Development}\label{further-development}}

This is meant to be a simple, generalised, first-principles model for
controlling the drivetrain. I hope it provides a suitable base from
which to build more advanced concepts such as traction control.

